Node Replication: Theory And Practice

We define and study a term calculus implementing higher-order node replication. It is used to specify two different (weak) evaluation strategies: call-by-name and fully lazy call-by-need, that are shown to be observationally equivalent by using type theoretical technical tools.

==> proofs/U-stable-by-aprime.tex <==
 \begin{proof}
  An easy induction proves that $t \in \purelterms$ implies $t\msub{x}{p} \in
  \purelterms$ for any $x$ and pure term $p$.
  We show that $t' \in \purelterms$ by induction on the reduction relation.
  \begin{enumerate}
    \item First, the base cases.
      \begin{itemize}
        \item $t = \ctx\lc{(\lam x p)} t_0 \rrule\db \ctx\lc{p \es x {t_0}} = t'$. Since 
          $p, t_0 \in \purelterms$, then  $t' \in
          \purelterms$.
        \item $t = t_0 \es x {\ctx\lc y} \rrule\varrr \ctx\lc{t_0 \msub x y} = t'$. Since 
          $t_0 \in \purelterms$ and $y$ is pure then  $t' \in \purelterms$.
        \item $t = t_0 \es x {\ctx\lc{t_1t_2}} \rrule\apprr \ctx\lc{t_0 \msub x {yz} \es y {t_1} \es z {t_2}}$. Since
          $t_0 \in \purelterms$ and $yz$ is pure then  $t' \in \purelterms$.
        \item $t = t_0 \es x {\ctx\lc{\lam y p}} \rrule\distrr \ctx\lc{t_0 \dist x {\lam y {z \es z p}}} =t'$. Since
          $t_0 \in \purelterms$ and $\nbocc z z = 1$ then
          $\lam y {z \es z p} \in \llset$ and thus $t' \in \purelterms$.
        \item $t = t_0 \dist x {\lam y {\ctx\llc p}} \rrule\absrr \ctx\llc{t_0 \msub x {\lam y p}} =t'$. Since 
          $t_0 \in \purelterms$ and $\lam y p$ is pure then  $t' \in \purelterms$.
      \end{itemize}
    \item If $t = \lam x u$, then $t \in \purelterms$
      implies in particular that $u$ is pure, and then
      $u$  can only contain $\db$-redexes,
      so that $t$ does not $\nrep'$-reduce to any term $t'$.
    \item $t = t_0 u$ or $t = u t_0$ or $t = t_0 \cut x u$ or $t = u \es x
      {t_0}$ where $t' = t_0u$, $t' = ut_0$, $t' = t_0' \es x u$, or $t' = u \es
      x {t_0'}$ respectively, and $t_0 \rew{\nrep'} t_0'$.
      By hypothesis $t_0 \in \purelterms$, so by the \ih\ $t_0' \in \purelterms$ and thefore $t' \in \purelterms$.      .
    \item $t = u \dist x {t_0} \rew{\nrep'} u \dist x {t'_0} = t'$ where $t_0
      \rew\nrsub t_0'$.
      By hypothesis, $t_0 \in \llset$. By \autoref{l:t-stable}, $t'_0
      \in \llset$, then $t' \in \purelterms$.
      \qedhere
  \end{enumerate}
\end{proof}


==> proofs/se_flneed.tex <==
\begin{proof}
  By induction on the reduction relation. We present the
  base cases which are all the reductions at the root position, \ie\ for
  $\ndc=\ec$. Besides, similarly to the subject reduction proof, and
  w.l.o.g, we use \autoref{l:se_permlr} to only
  consider the case $\lc{} = \ec$ in the following rules.
  \begin{itemize}
    \item $t_0 = (\lam x t) u \rew{\db} t \es x u = t_1$. This case is the same
      as for $\rew\whlr$.

    \item $t_0 = \ctxnc\ndc x \es x {\lam y p} \rew\ndlrdist
      \ctx\llc{\ctxnc\ndc x \dist x {\lam y {p'}}} = t_1$,
      where $\lam y {z \es z p} \skelbs{}_\skelss \lam y {\ctx\llc{p'}}$.
      By \autoref{l:se_permlr} there is $\dem {\Phi_{t'_1}}
      \Gamma {\ctxnc\ndc x \dist x {\lam y {\ctx\llc{p'}}}} \sigma$ and
      it is of the form
      \[\inferrule*[right=\ruleCutR]{
          \dem {\Phi} {\Gamma';x:\MN}{\ctxnc\ndc x}{ \sigma}
          \\ \inferrule*[Right=\many]{
          (\dem {\Phi_i} {\Delta_i}{\lam y {\ctx\llc{p'}}}{ \sigma_i})_{\iI}}{
      \seq \Delta {\lam y {\ctx\llc{p'}}} \MN}}{
      \seq {\Gamma' + \Delta}{\ctxnc\ndc x \dist x {\lam y
  {\ctx\llc{p'}}}}{\sigma}} \]
  where $\Del = +_{\iI} \Del_i$ and $\MN = \mult{\sig_i}_{\iI}$ where, by \autoref{l:typed-in-ndc}, $\MN \neq \emult$.
  Then, for each $\iI$ we have by \autoref{l:se_nrsub}
  that $\dem {\Phi'_i} {\Delta_i}{\lam y {z \es z p} }{ \sigma_i}$ which has
  two different shapes, depending on $\sig_i$.
  \begin{enumerate}
    \item If $\sig_i = \MM_i \ft \tau_i$ then $\Phi'_i$ is of the form:
      \[\inferrule*[right=\ruleAbsR]{
          \inferrule*[Right=\ruleCutR]{
            \inferrule*[right=\ruleAxR]{ }{\seq{z:\mult{\tau_i}}{z}{\tau_i}}
          \\ \dem {\Phi_p^i} {\Delta_i;y:\MM_i}{p}{\tau_i}}{
      \seq{\Delta_i;y:\MM_i}{z \es z p}{\tau_i}}}{
  \seq{\Delta_i}{\lam y {z \es z p}}{\MM_i \ft \tau_i}} \]
  Therefore we have $\Psi_i$ of the form \[\inferrule*[right=\ruleAbsR]{
    \dem {\Phi_p^i} {\Delta_i;y:\MM_i}{p}{\tau_i}}{
\seq{\Delta_i}{\lam y p }{\MM_i \ft \tau_i}} \]
\item If $\sigma_i = \ans$ then $\Del_i = \emptyset$ and we obtain $\Psi_i$ of the form
  $\inferrule*[right=\ruleAnsR,vcenter]{ }{\seq{}{\lam y p}{\ans}}$.
\end{enumerate}
We can then construct $\Phi_{t_0}$ as follows
\[\inferrule*[right=\ruleCutR]{
    \dem {\Phi} {\Gamma';x:\MN}{\ctxnc\ndc x}{ \sigma}
    \and \inferrule*[Right=\many]{
    (\dem {\Psi_i} {\Delta_i}{\lam y p}{ \sigma_i})_{\iI}}{
\seq \Delta {\lam y p}{ \MN}}}{
\seq {\Gamma' + \Delta}{\ctxnc\ndc x \es x {\lam y p}}{\sigma}} \]

\item $t_0 = \ctxnc\ndc x \dist x v \rew\ndlrabs \ctxnc\ndc v \dist x v = t_1$. Then $\Phi_{t_1}$ is of the form
  \[ \inferrule*[right=\ruleCutR]{
      \dem {\Phi} {\Gamma';  x:\MN'} {\ctxnc\ndc v}{\sigma} \\
    \dem {\Phi'_{v}} {\Del'}{v}{\MN'}}
  {\seq{\Gamma' + \Del'}{\ctxnc\ndc v \dist x v}{\sigma}} \]
  By \autoref{l:partial-anti-substitution} $\exists \Gam''$,
  $\exists\Del''$, $\exists\MN''$, $\exists\Phi'$,  $\exists \Phi''_v$
  s.t. $\Gamma';  x:\MN = \Gam'' + \Del'$, $\dem {\Phi'} {\Gam'' +
  x:\MN''}{\ctxnc\ndc x}{ \sigma}$ and $\dem {\Phi''_v} {\Delta''} {v}{
  \MN''}$. From $x \notin \fv v$ and the Relevance \autoref{l:relevance} we
  have that $x \notin \dom{\Del''}$. Thus $\Gam'' = \Gam'''; x:\MN'$ and then
  $\Gam'' + x:\MN' = \Gam''';x:\MN$ where $\MN = \MN' \sqcup \MN''$. From $\Phi'_v$
  and $\Phi''_v$ derivations we obtain $\dem {\Phi_v} {\Delta} {v}{
  \MN}$, where $\Delta = \Del' + \Del'' $. Then $\Phi_{t_0}$ is of the form:
  \[\inferrule*[right=\ruleCutR]{
      \dem {\Phi'} {\Gamma'''; x: \MN}{\ctxnc\ndc x}{\sigma}
    \and \dem {\Phi_v} {\Delta}{v}{\MN}}{
\seq{\Gamma''' + \Delta }{\ctxnc\ndc x \dist x v}{\sigma}} \]
where $\Gamma''' + \Delta = \Gam' + \Del'$.

\item The inductive cases are similar to those of subject reduction.
  \qedhere
\end{itemize}
\end{proof}


==> proofs/se_ndb.tex <==
\begin{proof}
  \loic{Note: in the appendix of the old long version, we don't present the
  inductive cases.}

  We reason by induction on the reduction relation $\rew\whdblr$.
  \begin{itemize}
    \item If $t_0 = (\lam x t) u \rew{\db} t \es x u = t_1$.
      Then $\Phi_{t_1}$ is of the form:
      \[ \inferrule*[right=\ruleCutR]{\dem {\Phi_t} {\Gamma'; x:\MM}{t}{ \sigma} \\
      \dem {\Phi_u} {\Gamma_u}{u }{ \MM}}
      {\seq{\Gamma' +  \Gamma_u}{ t\es x u}{ \sigma} } \]
      Therefore, we construct $\Phi_{t_0}$ as follows:
      \[\inferrule*[right=\ruleAppR]{
        \inferrule*[right=\ruleAbsR]{
          \dem {\Phi_t} {\Gamma'; x:\MM}{t}{ \sigma}}{
          \seq{\Gamma'}{\lam x t}{ \MM \ft \sigma}}
        \\ \dem {\Phi_u} {\Gamma_u}{u }{ \MM}}{
        \seq{\Gamma' +  \Gamma_u}{ (\lam x t)u}{ \sigma}} \]

    \item If $t_0 = tu \rew{\whdblr} t'u = t_1$, where $t \rew{\whdblr} t'$, then
      the property trivially holds by the \ih

    \item If $t_0 = t \es x u \rew{\whdblr} t' \es x u = t_1$, where $t \rew{\whdblr} t'$, then $\Gamma = \cmin{\Gamma'}{x} + \Delta$ and
      $\dem {\Phi_t} {\Gamma';x:\MM}{t}{\sigma}$
      and $\dem {\Phi_u} {\Delta}{u }{\MM}$.
      By the \ih\ we have
      $\dem {\Phi_{t'}} {\Gamma';x:\MM}{t'}{\sigma}$.
      Derivation $\Phi_{t_1}$ is then
      obtained by rule $\ruleCutR$ from $\Phi_{t'} $ and $\Phi_u$.
      \qedhere
  \end{itemize}
\end{proof}


==> proofs/se_nrsub.tex <==
\begin{proof}
  Since $t_0 \rew{\nrsub} t_1$ implies $t_0 \rewn{\permlr}
  t' \rew{\purelr\nrsub} t_1$ for some
  $t'$, we prove the property for $\rew{\purelr\nrsub}$ and conclude by applying
  \autoref{l:se_permlr}.

  Let $t' = \ctx{\fc}{t'_0}$ and $t_1 = \ctx{\fc}{t'_1}$, where  $t'_0
  \rew{\purelr\nrsub} t'_1$ is a root reduction, and $\dem {\Phi_{t_1}} \Gamma
  {t_1}{\sigma}$.
  First, we consider the base cases, \ie\, when $\fc = \ec$:
  \begin{itemize}
    \item  $t' = t \es {x} {us}  \rew{\purelr\nrsub}  {t \msub {x} {yz} \es y
      u \es z s} = t_1$.
      Then $\Phi_{t_1}$ is of the form:
      \[\inferrule*{ \inferrule*{ \dem {\Phi} {\Gam';z:\MN_s;y:\MN_u}{t \msub {x} {yz}}{
            \sig} \\ \dem {\Phi_u} {\Del_u}{u}{\MN_u}}{\seq{(\Gam' + \Del_u);z:\MN_s}{t
        \msub {x} {yz} \es y u}{\sig}} \\ \dem {\Phi_s} {\Del_s}{s}{\MN_s}}{\seq{\Gam' +
  \Del_u + \Del_s}{t \msub {x} {yz} \es y u \es z s}{ \sig}}\]
  where $\Gam = \Gam' + \Del_u + \Del_s$. Also $(\Gam' ;z:\MN_s) + \Del_u =
  (\Gam' + \Del_u);z:\MN_s$ since $z \notin \dom{\Del_u}$ by the Relevance \autoref{l:relevance}.
  By \autoref{l:anti-substitution} $\exists \Gam''$,
  $\exists \Del$, $\exists \MM$, $\exists \Phi'$,  $\exists \Phi_{yz}$ s.t.
  $\Gam';z:\MN_s;y:\MN_u = \Gam'' + \Del$, $\dem {\Phi'} {\Gam'';x:\MM}{t}{
  \sigma}$ and $\dem {\Phi_{yz}} \Delta {yz} \MM$. By freshness of $y,z$ and
  \autoref{l:relevance} we have that $y,z \notin \dom{\Gam''} \cup \{x\}$.
  Then $\Gam'' = \Gam'$ and $\Del = z:\MN_s;y:\MN_u$. From $\Phi_{yz}$,
  $\Phi_u$, $\Phi_s$ and \autoref{l:partial-substitution} we obtain $\dem
  {\Phi_{us}} {\Del_u + \Del_s}{us}{\MM}$ and construct $\Phi_{t'}$ as:
  \[\Phi_{t'} = \inferrule{\dem {\Phi'} {\Gam';x:\MM}{t}{ \sigma} \\ \dem {\Phi_{us}}
  {\Del_u + \Del_s}{us}{\MM}}{\seq{\Gam' + \Del_u + \Del_s}{t \es {x} {us}}{\sig}}\]

\item $t' =  t \es {x} {\lam y u}  \rew{\purelr\nrsub}  {t \dist {x} {\lam y z \es
  {z} u}} = t_1$.
  Then $\Phi_{t_1}$ is of the form:
  \[\inferrule*{ \dem {\Phi_t} {\Gam_t;x:\mult{\tau_i}_{\iI}}{t}{\sig} \\
      \inferrule*{(\dem {\Phi_i} {\Del_i}{\lam y z \es z u }{
        \tau_i})_{\iI}}{\seq{\Del}{\lam y z \es z u  }{
  \mult{\tau_i}_{\iI}}}}{\seq{\Gam_t + \Del}{t \dist x {\lam y z \es z u}}{ \sig}}\]
  where $\Del = +_{\iI} \Del_i$ and $\Gam = \Gam_t + \Del$. There are two possibilities for each $\Phi_i$, depending on $\tau_i$:
  \begin{enumerate}
    \item If $\tau_i = \MN_i \ft \sig_i$ then $\Phi_i$ is of the form:
      \[\inferrule{ \inferrule*{ }{\seq{z:\mult{\sig_i}}{z}{\sig_i}} \\
          \inferrule*{\dem {\Phi_u^i}
        {\Del_i;y:\MN_i}{u}{\sig_i}}{\seq{\Del_i;y:\MN_i}{u}{\mult{\sig_i}}}}{\inferrule{
  \seq{\Del_i;y:\MN_i}{z \es z u}{ \sig_i} }{\seq{\Del_i}{\lam y z \es z u }{ \MN_i \ft \sig_i}}}\]
  We then construct
  \[\Phi'_i = \inferrule{\dem {\Phi_u^i}
  {\Del_i;y:\MN_i}{u}{\sig_i}}{\seq{\Del_i}{\lam y u}{\MN_i \ft \sig_i}}\]

\item If $\tau_i = \ans$ then $\Del_i = \emptyset$ and we construct
  $\Phi'_i = \inferrule{ }{\seq{ }{\lam y u}{\ans}}$  
\end{enumerate}

Then we construct $\Phi_{t'}$ as follows:
\[\Phi_{t'} = \inferrule{ \dem {\Phi_t} {\Gam_t;x:\mult{\tau_i}_{\iI}}{t}{\sig} \\
    \inferrule{\left( \dem {\Phi'_i} {\Del_i}{\lam y u}{ \tau_i}
  \right)_{\iI}}{\seq{\Del}{\lam y u}{\mult{\tau_i}_{\iI}}} }{\seq{\Gam_t +
\Del}{t \es x {\lam y u}}{ \sig}}\]

\item $t' =  t \dist x {\ly.p}   \rew{\purelr\nrsub}   {t \msub {x} {\lam y p}} = t_1$ then by
  \autoref{l:anti-substitution}  $\exists \Gam'$,
  $\exists \Del$, $\exists \MM$, $\exists \Phi'$,  $\exists \Phi_{\lam y p}$
  s.t. $\Gam = \Gam' + \Del$, $\dem {\Phi'} {\Gam';x:\MM}{t}{ \sigma}$
  and $\dem {\Phi_{\lam y p}} \Delta {\lam y p}{ \MM}$. Therefore:
  \[\Phi_{t'} = \inferrule
    {\dem {\Phi'} {\Gam';x:\MM}{t}{ \sigma}
    \and \dem {\Phi_{\lam y p}} \Delta {\lam y p}{\MM}}
  {\seq{\Gam' + \Del}{t \dist {x} {\lam y p}}{\sig}}\]

\item $t' =  t \es {x} {y} \rew{\purelr\nrsub}  {t \msub {x} y} = t_1$  then
  $\Phi_{t'}$ is obtained similarly to the previous case.
\end{itemize}

We then proceed with  the inductive steps:
\begin{itemize}
  \item $t' = \lam x \ctx{\fc}{t'_0} \rew{\purelr\nrsub} \lam x \ctx{\fc}{t'_1} = t_1$ then  there are two possibilities for $\Phi_{t_1}$ depending on $\sigma$:
    \begin{enumerate}
      \item If $\sig = \MN \ft \tau$ then $\Phi_{t_1}$ is of the form:
        \[\inferrule
          {\dem {\Phi_\fc}{\Gam;x:\MN}{\ctx{\fc}{t'_1}} \tau}
          {\seq \Gamma {\lam x {\ctx{\fc}{t'_1}}}{\MN \ft \tau}}\]
        Then by the \ih\ we have $\dem {\Phi'_\fc}
        {\Gam;x:\MN}{\ctx{\fc}{t'_0}}{\tau}$ and we construct
        \[\Phi_{t'} = \inferrule{\dem{\Phi'_\fc}
            {\Gam;x:\MN}{\ctx{\fc}{t'_0}}{\tau}}{\seq{\Del}{\lam x
        {\ctx{\fc}{t'_0}}}{\MN \ft \tau}}\]

      \item If $\sig = \ans$ then $\Gam = \emptyset$ and we construct
        $\Phi_{t'} = \inferrule*{ }{\seq{ }{\lam x {\ctx{\fc}{t'_0}}}{\ans}}$ 
    \end{enumerate}

  \item $t' = \ctx{\fc}{t'_0} t \rew{\purelr\nrsub} \ctx{\fc}{t'_1} t = t_1$ then  $\Phi_{t_1}$ is of the form:
    \[\inferrule
      {\dem {\Phi_\fc} {\Gam_\fc}{\ctx{\fc}{t'_1}}{\MN \ft \sigma}
      \and \dem {\Phi_t} {\Gam_t} t \MN}
    {\seq{\Gamma_\fc + \Gamma_t}{\ctx{\fc}{t'_1} t}{\sigma}}\]
      Then by the \ih\ we have $\dem {\Phi'_\fc}
      {\Gam_{\fc}}{\ctx{\fc}{t'_0} }{ \MN \ft \sig}$ and we obtain $\Phi_{t'}$ as:
      \[\inferrule
        {\dem{\Phi'_\fc} {\Gam_{\fc}}{\ctx{\fc}{t'_0} }{\MN \ft \sig}
          \and \dem {\Phi_t} {\Gam_t}{t}{\MN}}
        {\seq{\Gam_{\fc} + \Gam_t}{\ctx{\fc}{t'_0} t}{\sig}}\]

      \item $t' = t \ctx{\fc}{t'_0}  \rew{\purelr\nrsub} t \ctx{\fc}{t'_1} = t_1$ then  $\Phi_{t_1}$ is of the form:
        \[\inferrule*{ \dem {\Phi_t} {\Gam_t}{t}{\mult{\tau_i}_{\iI} \ft \sig} \\
            \inferrule*{(\dem {\Phi_i} {\Del_i}{\ctx{\fc}{t'_1} }{
              \tau_i})_{\iI}}{\seq{\Del}{\ctx{\fc}{t'_1}  }{
        \mult{\tau_i}_{\iI}}}}{\seq{\Gam_t + \Del}{t \ctx{\fc}{t'_1}}{ \sig}}\]
        where $\Del = +_{\iI} \Del_i$ and $\Gam = \Gam_t + \Del$. Then by \ih\ we
        have $\dem {\Phi'_i} {\Del_i}{\ctx{\fc}{t'_0} }{ \tau_i}$, for each $\iI$. Finally, we construct $\Phi_{t'}$:
        \[\inferrule*{ \dem {\Phi_t} {\Gam_t}{t}{\mult{\tau_i}_{\iI} \ft \sig} \\
            \inferrule*{(\dem {\Phi'_i} {\Del_i}{\ctx{\fc}{t'_0} }{
              \tau_i})_{\iI}}{\seq{\Del}{\ctx{\fc}{t'_0}  }{
        \mult{\tau_i}_{\iI}}}}{\seq{\Gam_t + \Del}{t \ctx{\fc}{t'_0}}{ \sig}}\]

      \item $t' = \ctx{\fc}{t'_0}  \cut x t  \rew{\purelr\nrsub} \ctx{\fc}{t'_1}  \cut x t = t_1$ then  $\Phi_{t_1}$ is of the form:
        \[\inferrule
          {\dem {\Phi_\fc} {\Gam_{\fc}; x:\MN}{\ctx{\fc}{t'_1}} \sigma
            \and \dem {\Phi_t} {\Gam_t}{t}{\MN}}
          {\seq{\Gam_{\fc} + \Gam_t}{\ctx{\fc}{t'_1} \cut x t}{\sig}}\]
          Then by the \ih\ we have $\dem {\Phi'_\fc} {\Gam_{\fc};
          x:\MN}{\ctx{\fc}{t'_0}} \sigma$ and we obtain $\Phi_{t'}$ as:
          \[\inferrule{\dem{\Phi'_\fc} {\Gam_{\fc}; x:\MN}{\ctx{\fc}{t'_0}
                }{ \sig} \and \dem {\Phi_t} {\Gam_t}{t}{\MN}}{\seq{\Gam_{\fc} +
            \Gam_t}{\ctx{\fc}{t'_0} \cut x t}{\sig}}\]

          \item  $t' = t \cut x {\ctx{\fc}{t'_0}}  \rew{\purelr\nrsub} t \cut x {\ctx{\fc}{t'_1}} = t_1$ then  $\Phi_{t_1}$ is of the form:
            \[\inferrule*{ \dem {\Phi_t} {\Gam_t;x:\mult{\tau_i}_{\iI}}{t}{\sig} \\
                \inferrule*{(\dem {\Phi_i} {\Del_i}{\ctx{\fc}{t'_1} }{
                  \tau_i})_{\iI}}{\seq{\Del}{\ctx{\fc}{t'_1}  }{
            \mult{\tau_i}_{\iI}}}}{\seq{\Gam_t + \Del}{t \cut x {\ctx{\fc}{t'_1}}}{ \sig}}\]
            where $\Del = +_{\iI} \Del_i$ and $\Gam = \Gam_t + \Del$.  Then by \ih\ we
            have $\dem {\Phi'_i} {\Del_i}{\ctx{\fc}{t'_0} }{ \tau_i}$, for each $\iI$. Finally, we construct $\Phi_{t'}$:
            \[\inferrule*{\dem {\Phi_t} {\Gam_t;x:\mult{\tau_i}_{\iI}}{t}{\sig} \\
                \inferrule*{(\dem {\Phi'_i} {\Del_i}{\ctx{\fc}{t'_0} }{
                  \tau_i})_{\iI}}{\seq{\Del}{\ctx{\fc}{t'_0}  }{
            \mult{\tau_i}_{\iI}}}}{\seq{\Gam_t + \Del}{t \cut x
      {\ctx{\fc}{t'_0}}}{ \sig}} \qedhere\]
        \end{itemize}
      \end{proof}


==> proofs/se_permlr.tex <==
\begin{proof}
  Let $t_0 = \ctx{\fc}{t'_0}$ and $t_1 = \ctx{\fc}{t'_1}$,
  where $t'_0 \rew{\pi} t'_1$ is a root step.
  We reason by induction on $\fc$.
  We consider the base cases, where $\fc = \ec$. Note that, in all such case,
  $\Phi_{t_1}$ is of the form: \[\inferrule*[right=\ruleCutR]{\dem {\Phi_{t'}}
    {\Gamma';x:\MM}{t'}{ \sig} \\ \dem {\Phi_u} {\Delta_u}{u}{\MM}}{\seq{\Gamma' +
\Delta_u}{t' \cut x u}{ \sig}}\]
\begin{itemize}
  \item If $t_0 = \lam y {t \cut x u} \rew\pi (\lam y t) \cut x u =t_1$
    where $y \notin \fv{u}$, then $t' = \ly.t$ and there are two cases, depending on $\sig$:
    \begin{enumerate}
      \item If $\sig = \MN \ft \tau$ then $\Phi_{t'}$ is of the form
        \[\inferrule*[right=\ruleAbsR]{\dem {\Phi_t}
        {\Gamma';x:\MM;y:\MN}{t}{\tau}}{\seq{\Gamma';x:\MM}{\lam y t}{ \MN \ft \tau}}\]
        From $y \notin \fv{u}$ and \autoref{l:relevance} we have that $y \notin \dom{\Del_u}$ thus $(\Gamma';y:\MN) + \Del_u = (\Gamma' + \Del_u);y:\MN$. We then construct $\Phi_{t_0}$ as:
        \[\inferrule*[right=\ruleCutR]{ \dem {\Phi_t}
          {\Gamma';x:\MM;y:\MN}{t}{\tau} \\ \dem {\Phi_u} {\Delta_u}{u}{\MM}}{
          \inferrule*[right=\ruleAbsR]{\seq{(\Gamma' + \Del_u);y:\MN}{t \cut x
      u}{\tau}}{\seq {\Gamma' + \Del_u}{\lam y {t \cut x u}}{ \MN \ft \tau} }}\]

    \item If $\sig = \ans$ then
      $\Phi_{t'} = \infer{ }{\seq{}{\ly.t}\ans}$ and $\Phi_u = \infer{ }{\seq {}{u}{\emult}}$.
      We can then obtain
  $\Phi_{t_0} = \infer{ }{\seq{}{\ly.t \cut x u} \ans}$.  \end{enumerate}

\item If either $t_0 = t \cut x u s $ where $x \notin \fv{s}$ or $t_0 = t s \cut x u $ where $x \notin \fv{t}$ then $t_0 \rew\pi (ts) \cut x u = t_1$, $t' = (ts)$ and $\Phi_{t'}$ is of the form:
  \[\inferrule*[right=\ruleAppR]{\dem {\Phi_t} {\Gamma_t}{t}{\MN \ft \sigma}  \\
  \dem {\Phi_s} {\Gam_s}{s}{\MN}}{\seq{\Gamma_t +\Gam_s}{ts}{\sigma}}\]
  where $\Gam';x:\MM = \Gamma_t +\Gam_s$. We analyse the two cases, depending on $t_0$:
  \begin{enumerate}
    \item  If $t_0 = t \cut x u s $ where $x \notin \fv{s}$, then
      $x \notin \dom{\Gam_s}$ by \autoref{l:relevance} thus $\Gam_t = \Gam'_t; x:\MM$  where $\Gam' = \Gam'_t + \Gam_s$. We construct $\Phi_{t_0}$ as follows:
      \[\inferrule*[right=\ruleAppR]{\inferrule*[right=\ruleCutR]{\dem
            {\Phi_t} {\Gam'_t; x:\MM}{t}{\MN \ft \sigma} \\ \dem {\Phi_u}
          {\Delta_u}{u}{\MM}}{\seq{\Gam'_t + \Del_u}{t \cut x u }{\MN \ft \sigma}} \\
      \dem {\Phi_s} {\Gam_s}{s}{\MN}}{\seq{\Gam' + \Del_u}{ t \cut x u s }{ \sig}}\]

    \item  If  $t_0 = t s \cut x u $ where $x \notin \fv{t}$, then $x
      \notin \dom{\Gam_t}$ by \autoref{l:relevance}.
      Thus $\Gam_s = \Gam'_s; x:\MM$  where $\Gam' = \Gam_t + \Gam'_s$.
      From $\dem {\Phi_s} {\Gam'_s; x:\MM}{s}{\MN}$ and $\dem {\Phi_u}
      {\Delta_u}{u}{\MM}$ one obtains $\dem {\Psi} {\Gam'_s + \Del_u}{s
      \cut x u}{\MN}$. Therefore, we construct $\Phi_{t_0}$ as follows:
      \[\inferrule*[right=\ruleAppR]{\dem {\Phi_t} {\Gamma_t}{t}{\MN \ft
          \sigma} \\ \dem {\Psi} {\Gam'_s + \Del_u}{s \cut x
      u}{\MN}}{\seq{\Gam' + \Del_u}{ t s \cut x u }{ \sig}}\]
  \end{enumerate} 

\item If $t_0 = t \cut y {s \cut x u} \rew\pi t \cut y s \cut x u =t_1$
  where $x \notin \fv{t}$, then $t' = t \cut y s$ and $\Phi_{t'}$ is of the form:
  \[\inferrule*[right=\ruleCutR]{\dem {\Phi_{t}} {\Gamma_t;y:\MN}{t}{ \sig}
  \\ \dem {\Phi_s} {\Gam_s}{s}{\MN}}{\seq{\Gamma_t + \Gam_s}{t \cut y s}{ \sig}}\]
  where $\Gamma';x:\MM = \Gam_t + \Gam_s$.  From $x \notin \fv{t}$ and
  \autoref{l:relevance} we have that $x \notin \dom{\Gam_t} \cup \{y\}$
  thus $\Gam_s = \Gam'_s; x:\MM$ where $\Gam' =\Gam_t + \Gam'_s$. From
  $\dem {\Phi_s} {\Gam'_s; x:\MM}{s}{\MN}$ and $\dem {\Phi_u}
  {\Delta_u}{u}{\MM}$ one obtains $\dem {\Psi} {\Gam'_s + \Del_u}{s \cut x
  u}{\MN}$. Therefore, we construct $\Phi_{t_0}$ as follows:
  \[\inferrule*[right=\ruleCutR]{\dem {\Phi_t} {\Gam_t;y: \MN}{t}{\sigma} \\
      \dem {\Psi} {\Gam'_s + \Del_u}{s \cut x u}{\MN}}{\seq{\Gam' + \Del_u}{ t
  \cut y {s \cut x u} }{ \sig}}\]
\end{itemize}

The analysis of all inductive cases w.r.t. $\fc$ proceeds similarly to the subject reduction proof. 
\end{proof}


==> proofs/simul-lr-es.tex <==
\begin{proof}
  The proofs of the corresponding stated relations are by induction on them.
  \begin{enumerate}
    \begin{item}
      If $t \rew\permlr t'$, then $t = \ctx\fc{t_0} \rew\permlr \ctx\fc{t_1} = t'$,
      where $t_0 \rew\permlr t_1$ is a root step.
      If $\fc = \ec$ we have the following cases:
      \begin{itemize}
        \item $\maprl {(\lam y {t \cut x u)}}
          = \lam y {\maprl t \msub x {\maprl u}}
          = (\lam y \maprl t) \msub x {\maprl u}
          = \maprl {((\lam y t) \cut x u)}$
        \item $\maprl {(t \cut x u v)}
          = \maprl t \msub x {\maprl u} \maprl v
          = (\maprl t \maprl v) \msub x {\maprl u}
          = \maprl {((tv) \cut x u)}$
        \item $\maprl {(tv \cut x u)}
          = \maprl t \maprl v \msub x {\maprl u}
          = (\maprl t \maprl v) \msub x {\maprl u}
          = \maprl {((tv) \cut x u)}$
        \item $\maprl {(t \cut y {v \cut x u)}}
          = \maprl t \msub y {\maprl v \msub x {\maprl u}}
          = \maprl t \msub y {\maprl v} \msub x {\maprl u}
          = \maprl {(t \cut y v \cut x u)}$
      \end{itemize}
      For the inductive cases, we reason as follows.
      \begin{itemize}
        \item If $\fc = \lam x \fc'$, then
          $\maprl {(\lam x {\ctx{\fc'} {t_0}})}
          = \lam x \maprl {(\ctx{\fc'} {t_0})}
          =_\ih \lam x \maprl {(\ctx{\fc'}{t_1})}
          = \maprl {(\lam x \ctx{\fc'}{t_1})}.$
        \item If $\fc = \fc' u$, then
          $\maprl {(\ctx{\fc'} {t_0} u)}
          = \maprl {(\ctx{\fc'} {t_0})} \maprl u
          =_\ih \maprl {(\ctx{\fc'}{t_1})} \maprl u
          = \maprl {(\ctx{\fc'}{t_1} u)}.$
        \item If $\fc = u \fc'$, then
          $\maprl {(u \ctx{\fc'} {t_0})}
          = \maprl u \maprl {(\ctx{\fc'} {t_0})}
          =_\ih \maprl u \maprl {(\ctx{\fc'}{t_1})}
          = \maprl {(u \ctx{\fc'}{t_1})}.$
        \item If $\fc = \fc' \cut x u$, then
          $\maprl {(\ctx{\fc'} {t_0} \cut x u)}
          = \maprl {(\ctx{\fc'} {t_0})} \msub x {\maprl u}
          =_\ih \maprl {(\ctx{\fc'}{t_1})} \msub x {\maprl u}
          = \maprl {(\ctx{\fc'}{t_1} \cut x u)}.$
        \item If $\fc = u \cut x {\fc'}$, then
          $\maprl {(u \cut x {\ctx{\fc'} {t_0}})}
          = \maprl u \msub x {\maprl {(\ctx{\fc')} {t_0}}}
          =_\ih \maprl u \msub x {\maprl {(\ctx{\fc'}{t_1})}}
          = \maprl {(u \cut x {\ctx{\fc'}{t_1}})}.$
      \end{itemize}
    \end{item}

    \begin{item} If $t \rew\nrsub t'$,
      then $t = \ctx\fc {t_0} \rew\nrsub \ctx\fc{t_1} = t'$,
      where  $t_0 \rew\nrsub t_1$ is a root step. We first consider $\fc=\ec$.
      Let us call $\sig_\lc$ the substitution resulting
      from translating the list context $\lc$.
      We use the last point on $\permlr$ to push out list contexts in these
      equations.
      \begin{itemize}
        \item Case $t_0 = t \es x {\ctx \lc {uv}} \rew{}
          \ctx \lc { t \msub x {yz} \es y u \es z v}= t_1$.
          Then, $\maprl {(t \es x {\ctx \lc {uv}})}
          = \maprl {(\ctx \lc {t \es x { {uv}}})}
          = \sig_\lc (\maprl t \msub x {\maprl u \maprl v})
          = \sig_\lc (\maprl t \msub x {yz} \msub y {\maprl u} \msub z {\maprl v})
          = \sig_\lc (\maprl {( t \msub x {yz} \es y u \es z v)})
          =  \maprl {(\ctx \lc { t \msub x {yz} \es y u \es z v})}$.
        \item Case $t_0 = t \es x {\ctx \lc {\lam y u}} \rew{}
          \ctx \lc {t \dist x {\lam y {z \es z u}}} = t_1$. Then,
          $\maprl {(t \es x {\ctx \lc {\lam y u}})}
          = \maprl {(\ctx \lc {t \es x {\lam y u}})}
          = \sig_\lc (\maprl t \msub x {\lam y \maprl u})
          = \sig_\lc (\maprl t \msub x {\lam y {z \msub z {\maprl u}}})
          = \sig_\lc (\maprl {(t \dist x {\lam y {z \es z u}})})
          = \maprl {(\ctx \lc {t \dist x {\lam y {z \es z u}}})}$.
        \item Case $t_0 =  {t \dist x {\lam y u}} \rew{}
          \ctx \lc {t \msub x {\lam y {u'}}} = t_1$, where $u \rew\permlr
          \ctx \lc {u'}$ and $u'$ pure. Then
          $\maprl {(t \dist x {\lam y u})}
          = \maprl {( t \dist x {\ctx \lc {\l y. u'}})}
          = \maprl {(\ctx \lc {t \dist x {\lam y {u'}}})}
          = \sig_\lc (\maprl t \msub x {\lam y {\maprl {u'}}})
          = \sig_\lc (\maprl {(t \msub x {\lam y {u'}})})
          = \maprl {(\ctx \lc {t \msub x {\lam y {u'}}})}$.
        \item Case $t_0 =  t \es x {\ctx \lc y} \rew{}
          \ctx \lc {t \msub x y}= t_1$. Then
          $\maprl {(t \es x {\ctx \lc y})}
          = \maprl {(\ctx \lc  {t \es x y})}
          = \sig_\lc (\maprl {(t \es x y)})
          = \sig_\lc (\maprl t \msub x y)
          = \sig_\lc (\maprl {(t \msub x y)})
          = \maprl {(\ctx \lc {t \msub x y})}$.
      \end{itemize}
      The proof of the inductive cases is similar to the previous case.
    \end{item}

  \item If $t \rew\db t'$,
    then $t = \ctx\fc {t_0} \rew\db \ctx\fc{t_1} = t'$,
    where $t_0 \rew\db t_1$ is a root step.
    We first consider $\fc = \ec$.
    As before, $\sig_\lc$ is the substitution resulting from translating
    the list context $\lc$.\\
    Then we have $\maprl {(\ctx\lc{\lam x t} u)}
    = \sig_\lc (\maprl {((\lam x t) u)})
    = \sig_\lc ((\lam x \maprl t) \maprl u)
    \rew\beta \sig_\lc (\maprl t \msub x {\maprl u})
    = \sig_\lc (\maprl {(t \es x u)})
    = \maprl {(\ctx\lc{t \es x u})}$\\
    For the inductive cases, we reason as follows.
    \begin{itemize}
      \item If $\fc = \lam x \fc'$, then
        $\maprl {(\lam x {\ctx{\fc'}{t_0}})}
        = \lam x \maprl {(\ctx{\fc'}{t_0})}
        \rew\ih \lam x \maprl {(\ctx{\fc'}{t_1})}
        = \maprl {(\lam x \ctx{\fc'}{t_1})}.$
      \item If $\fc = \fc' u$, then
        $\maprl {(\ctx{\fc'} {t_0} u)}
        = \maprl {(\ctx{\fc'} {t_0})} \maprl u
        \rew\ih \maprl {(\ctx{\fc'}{t_1})} \maprl u
        = \maprl {(\ctx{\fc'}{t_1} u)}.$
      \item If $\fc = u \fc'$, then
        $\maprl {(u \ctx{\fc'} {t_0})}
        = \maprl u \maprl {(\ctx{\fc'} {t_0})}
        \rew\ih \maprl u \maprl {(\ctx{\fc'}{t_1})}
        = \maprl {(u \ctx{\fc'}{t_1})}.$
      \item If $\fc = \fc' \cut x u$, then
        $\maprl {(\ctx{\fc'} {t_0} \cut x u)}
        = \maprl {(\ctx{\fc'} {t_0})} \msub x {\maprl u}
        \rew\ih \maprl {(\ctx{\fc'}{t_1})} \msub x {\maprl u}
        = \maprl {(\ctx{\fc'}{t_1} \cut x u)}.$
      \item If $\fc = u \cut x {\fc'}$, then:
        \begin{itemize}
          \item if $x \notin \fv u$:
            $\maprl {(u \cut x {\ctx{\fc'} {t_0}})}
            = \maprl u \msub x {\ctx{\fc'} {t_0}}
            = \maprl u
            = \maprl {(u \cut x {\ctx{\fc'}{t_1}})}$,
          \item otherwise:
            $\maprl {(u \cut x {\ctx{\fc'} {t_0}})}
            = \maprl u \msub x {\ctx{\fc'} {t_0}}
            \rew\ih \maprl u \msub x {\ctx{\fc'}{t_1}}
            = \maprl {(u \cut x {\ctx{\fc'}{t_1}})}$.
            \qedhere
        \end{itemize}
    \end{itemize}
\end{enumerate}
\end{proof}


==> proofs/sr_redsub_full.tex <==
\begin{proof}
  As remarked in \autoref{sec:operational-semantics} $t_0 \rew \nrsub t_1$ implies
  $t_0  \rewn\permlr t' \rew{\purelr\nrsub} t_1$. By \autoref{l:sr_permlr},
  weighted subject reduction holds for
  $t_0  \rewn\permlr t'$, so  it is sufficient to show the statement for
  the relation $\rew{\purelr\nrsub}$. We reason by induction
  on this relation, first we consider the base cases.
  \begin{itemize}
    \item $t_0 = {t \es x {us}} \rew{\apprr} t \msub x {yz} \es y u \es
      z s = t_1$, where $y$ and $z$ are fresh variables.
      The typing derivation is of the form:
      \[ \Phi_{t_0} = \inferrule*[vcenter]{\dem {\Phi_t} {\Gam'; x:\MM}{t}{ \sig}
          \and \inferrule*{\left(\inferrule{\dem {\Phi^i_u} {\Gam^i_u}{u}{\MN_i  \ft  \rho_i}
              \and \dem {\Phi^i_s} {\Gam^i_s}{s}{\MN_i}}
          {\seq{\Gam^i_{u} + \Gam^i_{s}}{us }{ \rho_i}} \right )_{\iI} }
        {\seq{\Gam_u + \Gam_s}{us }{\MM}}}
      {\seq{\Gam'  +  \Gam_u + \Gam_s}{ t {\es x {us}}}{ \sig} } \]
      where $\MM = \mult{\rho_i}_{\iI}$,
      $\Gam_u  = +_{\iI} \Gam^i_u$ and $\Gam_s= +_{\iI} \Gam^i_s$.
      We have
      \begin{align*}
        \dermeasaux{\Phi_{t_0}} m
        &= \dermeasaux {\Phi_t} m\\
        &+ \sum_{\iI} \left(\dermeasaux {\Phi_u^i}{m + \lv x t + 1}
        + \dermeasaux {\Phi_s^i}{m + \lv x t +1} + (1, m + \lv x t + 1, 0)\right)
      \end{align*}

      Let us consider $\dem{\Phi'} {\Gam'; y:\MN_u; z:\MN_s}{ t \msub {x} {yz}}{ \sig}$,
      obtained by \autoref{l:qsub} from $\Phi_t$ and
      $\dem {\Phi_{yz}} {y:\MN_u; z:\MN_s}{yz}{ \mult{\rho_i}_{\iI}}$,
      where $\MN_u = \mult{\MN_i  \ft  \rho_i}_{\iI}$ and $\MN_s = \multunion_{\iI} \MN_i$.

      We construct the following derivation $\Phi_{t_1}$.
      \[
        \inferrule*{\inferrule*{
            \dem {\Phi'} {\Gam'; z:\MN_s; y:\MN_u}{ t \msub {x} {yz}}{ \sig} \\
          \inferrule*{(\dem{\Phi^i_u} {\Gam^i_u}{u}{\MN_i  \ft  \rho_i}
        )_{\iI}}{\seq{\Gam_u}{u}{\MN_u}}}
          { \seq{(\Gam'; z:\MN_s) + \Gam_u} {t \msub {x} {yz} \es y
          u}{\sig}} \and
        \inferrule*{(\dem{\Phi^i_s}{\Gam^i_s}{s}{\MN_i})_{\iI}}{\seq{\Gam_s}{s}{\MN_s}} }
      {\seq{\Gam'+\Gam_u+\Gam_s}{t \msub {x} {yz} \es y u \es z s}{\sig}} \]

      We consider two cases to conclude:
      \begin{itemize}
        \item If $\MM = \emult$, then
          \begin{align*}
            \dermeasaux {\Phi_{t_1}} m
             &= \dermeasaux {\Phi'} m + \sum_{\iI} \dermeasaux{\Phi_u^i}{m + \lv y {t \msub
             x {yz}} + 1} + \sum_{\iI} \dermeasaux{\Phi_s^i}{m + \lv z {t \msub x
         {yz} \es y u} + 1} \\
             &= \dermeasaux {\Phi'} m
             =_{\ref{l:qsub}} \dermeasaux {\Phi_t} m
             = \dermeasaux {\Phi_{t_0}} m
          \end{align*}
        \item If $\MM \neq \emult$, then
          \begin{align*}
            \dermeasaux {\Phi_{t_1}} m
            &= \dermeasaux {\Phi'} m + \sum_{\iI} \dermeasaux{\Phi_u^i}{m + \lv y {t \msub
            x {yz}} + 1} + \sum_{\iI} \dermeasaux{\Phi_s^i}{m + \lv z {t \msub x
        {yz} \es y u} + 1} \\
            & = \dermeasaux {\Phi'} m + \sum_{\iI} \dermeasaux{\Phi_u^i}{m + \lv y {t \msub x {yz}} + 1} + \sum_{\iI} \dermeasaux{\Phi_s^i}{m + \lv z {t \msub x {yz}} + 1} \\
            &=_{\ref{l:level-substitution}:\ref{l:level-substitution-non-void}} \dermeasaux{\Phi'} m + \sum_{\iI} \left(\dermeasaux{\Phi_u^i}{m+\lv x t + 1} + \dermeasaux{\Phi_s^i}{m + \lv x t + 1}\right) \\
            & \leq _{\ref{l:partial-substitution}} \dermeasaux{\Phi_t} m + \dermeasaux{\Phi_{yz}}{m + \lv
              x t} + \sum_{\iI} \left(\dermeasaux{\Phi_u^i}{m+\lv x t + 1} +
              \dermeasaux{\Phi_s^i}{m + \lv x t + 1}\right) \\
            & = \dermeasaux{\Phi_t} m + (1, m + \lv x t, 2) + \sum_{\iI}
            \left(\dermeasaux{\Phi_u^i}{m+\lv x t + 1} + \dermeasaux{\Phi_s^i}{m + \lv x
            t + 1} \right) \\
            & < \dermeasaux{\Phi_t} m + \sum_{\iI} \left(\dermeasaux{\Phi_u^i}{m+\lv x t + 1} + \dermeasaux{\Phi_s^i}{m + \lv x t + 1} + (1, m + \lv x t, 2)\right) \\
            &< \dermeasaux{\Phi_{t_0}} m.
          \end{align*}
      \end{itemize}

    \item $t_0 =  {t \es x {\lam y u}} \rew{\distrr} t \dist x {\lam y
      z \es z u} = t_1$.
      The typing derivation is of the form:
      \[ \Phi_{t_0} = \inferrule*[vcenter]{\dem {\Phi_t} {\Gam'; x:\MM} t \sigma \and
        \dem {\Phi_{\lam y u}} {\Gam_{\lam y u}}{\lam y u} \MM}
      {\seq{\Gam'  +  \Gam_{\lam y u}}{t {\es x {\lam y u}}} \sigma} \]
      where \[
        \Phi_{\lam y u} =
        \inferrule*[vcenter]{
          \left( \inferrule{ \dem {\Phi^i} {\Gam^i_{\lam y u}; y:\MN_i }{u}{\rho_i}}
          {\seq{\Gam^i_{\lam y u}}{\lam y u }{ \MN_i \ft \rho_i}} \right)_{\iI}
          \left( \inferrule{}
          {\seq{}{\lam y u}{ \ans}} \right)^k
        }{ \seq{\Gam_{\lam y u}}{\lam y u }{ \MM}}
      \]
      and $\MM = \mult{\MN_i \ft \rho_i}_{\iI} \multunion \mult{\underbrace{\ans,\dots,\ans}_{k}}$,
      with $\Gam_u = +_\iI \Gam^i_{\lam y u}$.
      Moreover, \[
      \dermeasaux{\Phi_{t_0}} m = \dermeasaux {\Phi_t} m + \sum_{\iI} \left(\dermeasaux {\Phi^i}{m + \lv x t + 1} + (1, m + \lv x t + 1, 0)\right) + k * (1, m + \lv x t + 1, 0). \]

      We construct the following derivation
      \[ \Phi_{t_1} = \inferrule*[vcenter]{\dem {\Phi_t} {\Gam'; x:\MM}{t}{ \sig} \and
        \dem {\Phi_\lambda} {\Gam_{\lam y u}}{\lam y z \es z u  }{ \MM }}
      {\seq{\Gam' + \Gam_{\lam y u}}{t \dist x {\lam y {z \es z u}}}{ \sig} } \]
      where \[
        \Phi_\lambda =
        \inferrule*[vcenter]{
          \left( \inferrule{ \inferrule*{ }{\seq{z:\mult{\rho_i}}{z}{\rho_i}}
              \and
            \dem{\Phi^i} {\Gam^i_{\lam y u}; y:\MN_i }{u}{\rho_i}}{
            \inferrule*{
            \seq{\Gam^i_{\lam y u}; y:\MN_i}{z \es z u}{ \rho_i}}{
        \seq{\Gam^i_{\lam y u}}{\lam y z \es z u }{ \MN_i \ft \rho_i}}}
      \right)_{\iI}
      \left( \inferrule{}
    {\seq{}{\lam y {z \es z u}}{ \ans}} \right)^k }{
\seq{\Gam_{\lam y u}}{\lam y z \es z u  }{ \MM}} \]

We have
\begin{align*}
  \dermeasaux{\Phi_{t_1}} m
        &= \dermeasaux{\Phi_t} m + \sum_{\iI} \left(\dermeasaux{\Phi^i}{m + \lv x t + 1} + (0,0,1) + (1,m+\lv x t,0)\right) + k * (1, m + \lv x t, 0) \\
        &\leq \dermeasaux{\Phi_{t_0}} m
\end{align*}
\item $t_0 = t \dist x {\lam y u} \rew\absrr t \msub x {\lam y
  u} = t_1$, where $u$ is pure.
  The derivation is of the form:
  \[ \Phi_{t_0} = \infer{\dem {\Phi_t} {\Gam'; x:\MM}{t}{ \sig} \and
    \dem {\Phi'} {\Gam_u}{\lam y u }{ \MM}}
  {\seq{\Gam' + \Gam_u}{t {\dist x {\lam y u}}}{ \sig} } \]
  Then, by \autoref{l:partial-substitution} we have
  $\dem {\Phi_{t_1}} {\Gamma' + \Gamma_u}{t \msub x {\lam y u}}{\sigma}$, where $\dermeasaux{\Phi_{t_1}} m \leq \dermeasaux{\Phi_t} m + \dermeasaux{\Phi'}{m + \lv x t} = \dermeasaux{\Phi_{t_0}} m$.

\item $t_0 = {t \es x y} \rew{\varrr} t \msub x y = t_1$.
  The derivation is of the form:
  \[ \Phi_{t_0} = \infer{\dem {\Phi_t} {\Gam'; x:\MM}{t}{ \sig} \and
    \dem {\Phi_y} {y:\MM}{y}{ \MM}}
  {\seq{\Gam' + y:\MM}{t \es x y}{ \sig}} \]
  By \autoref{l:partial-substitution} we have $\dem {\Phi_{t_1}} {\Gamma' +
  y:\MM}{t \msub x y}{\sigma}$, where $\dermeasaux{\Phi_{t_1}}
  m \leq \dermeasaux{\Phi_t} m + \dermeasaux{\Phi_y}{m + \lv x t} = \dermeasaux{\Phi_{t_0}} m$.

\end{itemize}

\noindent Now, the inductive cases. Let $t_0 = \ctx{\fc}{o} \rew{\purelr\nrsub}
\ctx{\fc}{o'} = t_1$, where $o \rew{\purelr\nrsub} o'$. We reason by cases. 

\begin{itemize}
  \item If $\fc = \lam x {\fc'}$, there are two cases.
    \begin{itemize}
      \item If $\sigma = \MM \ft \tau$,
        we have $\dem {\Phi} {\Gamma; x:\MM}{\ctx{\fc'} o}{\tau}$.
        By \ih\ there is $\dem {\Phi'} {\Gamma;x:\MM}{\ctx{\fc'}{o'}}{\tau}$.
        So $\dem {\Phi_{t_1}} \Gamma {\lam x {\ctx{\fc'}{o'}}}{\sigma}$.
        Moreover, $\dermeasaux{\Phi_{t_0}} m
        = \dermeasaux \Phi m + (1,m,0)
        \geq_\ih \dermeasaux{\Phi_{t_1}} m$.
      \item If $\sigma = \ans$,
        we have $\Gamma = \emptyset$ and
        $\dem {\Phi_{t_0}} {}{\lam x {\ctx{\fc'}{o}}}{\ans}$.
        We also have $\dem {\Phi_{t_1}} {}{\lam x {\ctx{\fc'}{o'}}}{\ans}$.
        Moreover, $\dermeasaux{\Phi_{t_0}} m
        = \dermeasaux{\Phi_{t_1}} m
        = (1,m,0)$.
    \end{itemize}
  \item If $\fc = \fc' u$, then
    we have $\Gamma = \Gamma' + \Delta$ and $\dem {\Phi} {\Gamma'}{\ctx{\fc'}o}{\MN \ft \sigma}$
    and $\dem {\Phi_u} {\Delta}{u}{\MN}$.
    By the \ih\ there is $\dem {\Phi'} {\Gamma'}{\ctx{\fc'}{o'}}{\MN \ft \sigma}$,
    so $\dem {\Phi_{t_1}} {\Gamma'+\Delta}{\ctx{\fc'}{o'}u}{\sigma}$.
    Moreover, $\dermeasaux{\Phi_{t_0}} m = \dermeasaux \Phi m + \dermeasaux{\Phi_u} m + (1,m,0) \geq_{\ih} \dermeasaux{\Phi'} m + \dermeasaux{\Phi_u} m + (1,m,0) = \dermeasaux{\Phi_{t_1}} m$.
  \item If $\fc = u \fc'$, then
    we have $\Gamma = \Gamma' +_{\iI} \Delta_i$ and $\dem {\Phi_u} {\Gamma'}{u}{\mult{\tau_i}_\iI \ft \sigma}$
    and $\dem {\Phi_i} {\Delta_i}{\ctx{\fc'} o }{\tau_i}$ for each $\iI$.
    By \ih\ there are $\dem {\Phi_i'} {\Delta_i}{\ctx{\fc'}{o'}}{\tau_i}$ for each $\iI$.
    So $\dem {\Phi_{t_1}} {\Gamma' +_\iI \Delta_i}{u \ctx{\fc'}{o'}}{\sigma}$.
    Moreover, $\dermeasaux{\Phi_{t_0}} m
    = \dermeasaux {\Phi_u} m + \sum_\iI \dermeasaux{\Phi_i} m + (1,m,0)
    \geq_{\ih} \dermeasaux{\Phi_u} m + \sum_\iI \dermeasaux{\Phi_i'} m + (1,m,0)
    = \dermeasaux{\Phi_{t_1}} m$.
  \item If $\fc = \fc \cut x u$, then
    we have $\Gamma = \Gamma' + \Delta$ and  $\dem {\Phi}
    {\Gamma';x:\MM}{\ctx{\fc'}o}{\sigma}$
    and $\dem {\Phi_u} {\Delta}{u}{\MM}$.
    By the \ih\ there is $\dem {\Phi'} {\Gamma';x:\MM}{\ctx{\fc'}{o'}}{\sigma}$,
    so $\dem {\Phi_{t_1}} {\Gamma'+\Delta}{\ctx{\fc'}{o'} \cut x u}{\sigma}$.
    Moreover, $\dermeasaux{\Phi_{t_0}} m = \dermeasaux \Phi m +
    \dermeasaux{\Phi_u}{m + \lv x{\ctx{\fc'}{o}} + \isES{\cut x u}}
    \geq_{\autoref{l:stability-levels}:\ref{l:stability-levels-substitution}}
    \dermeasaux \Phi m + \dermeasaux{\Phi_u}{m + \lv x{\ctx{\fc'}{o'}} +
    \isES{\cut x u}}
    \geq_{\ih} \dermeasaux{\Phi'} m + \dermeasaux{\Phi_u}{m + \lv x
    {\ctx{\fc'}{o'}} + \isES{\cut x u}}
    = \dermeasaux{\Phi_{t_1}} m$.
  \item If $\fc = u \cut x {\fc'}$, then
    we have $\Gamma = \Gamma' +_{\iI} \Del_i$ and $\dem {\Phi_u}
    {\Gamma';x:\mult{\tau_i}_\iI}{u}{\sigma}$
    and $\dem {\Phi_i} {\Delta_i}{\ctx{\fc'} o }{\tau_i}$ for each $\iI$.
    By \ih\ there are $\dem {\Phi_i'} {\Delta_i}{\ctx{\fc'}{o'}}{\tau_i}$ for each $\iI$.
    So $\dem {\Phi_{t_1}} {\Gamma' +_\iI \Delta_i}{u \cut x { \ctx{\fc'}{o'}}}{\sigma}$.
    Moreover, $\dermeasaux{\Phi_{t_0}} m
    = \dermeasaux {\Phi_u} m + \sum_\iI \dermeasaux{\Phi_i}{m + \lv x u +
    \isES{\cut x {\ctx{\fc'} o}}}
    \geq_{\ih} \dermeasaux{\Phi_u} m + \sum_\iI \dermeasaux{\Phi_i'}{m + \lv
    x u + \isES{\cut x {\ctx{\fc'}{o'}}}}
    = \dermeasaux{\Phi_{t_1}} m$.
    \qedhere
\end{itemize}
\end{proof}


==> proofs/sr_sw.tex <==
\begin{proof}
  The proof is by induction on $\Rew\redsubw $.
  First, it is easy to see that if $\Gamma = \emptyset$ and $\sigma = \ans$,
  we can type  $t_1$ through a proof $\dem {\Phi_{t_1}} {}{t_1}{\ans}$, which has the same measure as $\Phi_{t_0}$ for any $m$.
  From now on, let’s suppose $\sigma = \N \ft \tau$.
  We begin with the base rules $u_0 \rrule{}^y u_1$, which are the base
  cases of the induction reasoning.
  For all these rules, we have by hypothesis a derivation
  $\dem {\Phi_{u_0}} {\Gamma'}{u_0}{\tau}$.
  Let us consider   $d = \lv x {\ctxnc\ictx x} = \lv \ec \ictx$,
  because $x$ is a linear variable.
  We want to show that $\dem {\Phi_{u_1}} {\Gamma'}{u_1}{\tau}$ and that the measure decreases.
  \begin{itemize}
    \item $u_0 = \ctxnc\ictx x \es x y \rrule\varrr^y \ctxnc\ictx y = u_1$.
      The derivation is of the form:
      \[ \Phi_{u_0} =
      \inferrule*[right=(\cuttr)]{
        \dem {\Phi} {\Delta; x:\mult{\sigma_i}_{\iI}}{\ctxnc\ictx x}{ \tau}
        \\
        \inferrule*[right=(\many)]{
          \left( \inferrule{ }{\seq{y:\mult{\sigma_i}}{y}{\sigma_i}} (\ax)\right)_{\iI}}{
          \dem {\Phi_y} {y:\mult{\sigma_i}_{\iI}}{y}{\mult{\sigma_i}_{\iI}}}}{
        \seq{\Delta + y:\mult{\sigma_i}_{\iI}}{\ctxnc\ictx x \es x y}{\tau}} \]
      where $\Gam'=\Delta + y:\mult{\sigma_i}_{\iI}$.
      Then, by \autoref{l:partial-substitution} we have
      $\dem {\Phi_{u_1}} {\Delta + y:\mult{\sigma_i}_{\iI}}{\ctxnc\ictx y}{\tau}$, where $\dermeasaux{\Phi_{u_1}} m
      = \dermeasaux{\Phi} m + \dermeasaux{\Phi_y}{m + d} - (0,0,\ssz I)
      = \dermeasaux{\Phi} m
      \leq \dermeasaux{\Phi_{u_0}} m$.

    \item $u_0 = \ctxnc\ictx x \es x {pq} \rrule\apprr^y \ctxnc\ictx{x_1x_2} \es {x_1} p \es {x_2} q = u_1$,
      where $x_1$ and $x_2$ are fresh variables and $y \in \fv{pq}$.
      The typing derivation is of the form:
      \[ \Phi_{u_0} =
      \inferrule*[right=(\cuttr)]{
        \dem {\Phi} {\Delta; x:\M}{\ctxnc\ictx x}{ \tau}
        \\ \inferrule*[right=(\many)]{
          \left(\inferrule{\dem {\Phi^i_p} {\Gam^i_p}{p}{\N_i \ft \rho_i}
          \\ \dem {\Phi^i_q} {\Gam^i_q}{q}{\N_i}}{
            \seq{\Gam^i_p + \Gam^i_q}{pq }{ \rho_i}} \right)_{\iI}}{
          \seq{\Gam_p + \Gam_q}{pq }{ \M}}}{
        \seq{\Delta + \Gam_p + \Gam_q}{\ctxnc\ictx x \es x {pq}}{ \tau}} \]
      where $\Gam' = \Delta + \Gam_p + \Gam_q$, $\M = \mult{\rho_i}_{\iI}$,
      $\Gam_p  = +_{\iI} \Gam^i_p$ and $\Gam_q = +_{\iI} \Gam^i_q$.
      We have \[
        \dermeasaux{\Phi_{u_0}} m = \dermeasaux {\Phi} m + \sum_{\iI} \left(\dermeasaux {\Phi_p^i}{m + d + 1}
        + \dermeasaux {\Phi_q^i}{m + d +1} + (1, m + d + 1, 0)\right). \]

      By \autoref{l:partial-substitution}, we have
      $\dem {\Phi'} {\Delta;x_1:\N_p;x_2:\N_q}{\ctxnc\ictx{x_1x_2}}{ \tau}$
      obtained from $\Phi$ and
      \[ \Phi_{x_1x_2} =
      \inferrule*[right=(\many)]{
        \left( \inferrule{
          \inferrule*[right=(\ax)]{ }{
            \seq{x_1:\mult{\N_i \ft \rho_i}}{x_1}{\N_i \ft \rho_i}} \\
          \inferrule*[right=(\many)]{ }{\seq{x_2:\N_i}{x_2}{\N_i}}}{
          \seq{x_1:\mult{\N_i \ft \rho_i};x_2:\N_i}{x_1x_2}{\rho_i}}(\apptr)\right)_{\iI}}{
        \seq{x_1:\N_p;x_2:\N_q}{x_1x_2}{\mult{\rho_i}_{\iI}}} \]
      where  $\N_p = \mult{\N_i  \ft  \rho_i}_{\iI}$
      and $\N_q = \sqcup_{\iI} \N_i$.

      We construct the following derivation.
      \[ \Phi_{u_1} =
      \inferrule*{\inferrule*{
        \dem {\Phi'} {\Delta; x_2:\N_q; x_1:\N_p}{\ctxnc\ictx{x_1x_2}}{ \tau} \sep
        \inferrule*{(\seq{\dem {\Phi^i_p} ^i_p}{p}{\N_i  \ft  \rho_i}
      )_{\iI}}{\seq{\Gam_p}{p}{\N_p}}}
      { \seq{(\Delta; x_2:\N_q) + \Gam_p} {\ctxnc\ictx{x_1x_2} \es {x_1} p}{\tau}}\sep
      \inferrule*{(\seq{\dem {\Phi^i_q} ^i_q}{q}{\N_i})_{\iI}}{\seq{\Gam_q}{q}{\N_q}}}
      {\seq{\Delta+\Gam_p+\Gam_q}{\ctxnc\ictx{x_1x_2} \es {x_1} p \es {x_2}
  q}{\tau}} \]

      We have:
      \begin{align*}
        \dermeasaux {\Phi_{u_1}} m
        &= \dermeasaux {\Phi'} m + \sum_{\iI} \dermeasaux{\Phi_p^i}{m + \lv {x_1} {\ctxnc\ictx{x_1x_2}} + 1}
        + \sum_{\iI} \dermeasaux{\Phi_q^i}{m + \lv {x_2} {\ctxnc\ictx{x_1x_2} \es {x_1} p} + 1} \\
        &= \dermeasaux {\Phi'} m + \sum_{\iI}\left( \dermeasaux{\Phi_p^i}{m + d + 1}
        + \dermeasaux{\Phi_q^i}{m + d + 1} \right) \\
        &=_{\autoref{l:partial-substitution}} \dermeasaux \Phi m - (0,0,\ssz\M) + \dermeasaux{\Phi_{x_1x_2}}{m + d}
        + \sum_{\iI} \left( \dermeasaux{\Phi_p^i}{m + d + 1} + \dermeasaux{\Phi_q^i}{m + d + 1} \right) \\
        &= \dermeasaux \Phi m - (0,0,\ssz\M) + \sum_{\iI} (1, m+d, 1+\ssz{\N_i})
        + \sum_{\iI} \left( \dermeasaux{\Phi_p^i}{m + d + 1} + \dermeasaux{\Phi_q^i}{m + d + 1} \right) \\
        &= \dermeasaux \Phi m + \sum_{\iI} \left( (1, m+d, \ssz{\N_i})
        + \dermeasaux{\Phi_p^i}{m + d + 1} + \dermeasaux{\Phi_q^i}{m + d + 1} \right) \\
        &< \dermeasaux \Phi m + \sum_{\iI} \left((1, m+d+1, 0)
        + \dermeasaux{\Phi_p^i}{m + d + 1} + \dermeasaux{\Phi_q^i}{m + d + 1}\right) \\
        &= \dermeasaux{\Phi_{u_0}} m
      \end{align*}

    \item $u_0 =  t \es x {\lam z p} \rrule\distrr^y t \dist x {\lam z
      w \es w p} = u_1$.
      The typing derivation is of the form:
      \[ \Phi_{u_0} = \inferrule*{\dem {\Phi} {\Delta; x:\M}{t}{ \tau} \sep\sep
      \inferrule*{ \left( \inferrule{ \dem {\Phi^i} {\Gam^i_{\lam z p}; z:\N_i
          }{p}{\rho_i}}
      {\seq{\Gam^i_{\lam z p} }{\lam z p }{ \N_i \ft \rho_i}} \right)_{\iI} }
      {\seq{\Gam_{\lam z p}}{\lam z p }{ \M}}}
      {\seq{\Delta + \Gam_{\lam z p}}{t {\es x {\lam z p}}}{ \tau} } \]
      where $\Gam' = \Delta + \Gam_{\lam z p}$, $\M = \mult{\N_i \ft \rho_i}_{\iI}$
      and $\Gam_{\lam z p}  = +_{\iI} \Gam^i_{\lam z p}$. Moreover, \[
        \dermeasaux{\Phi_{u_0}} m = \dermeasaux {\Phi} m + \sum_{\iI} \left(\dermeasaux {\Phi^i}{m + \lv x t + 1} + (1, m + \lv x t + 1, 0)\right). \]

      We construct the following derivation
      \[ \Phi_{u_1} = \inferrule*{\dem {\Phi} {\Delta; x:\M}{t}{ \tau} \sep\sep
      \inferrule*{\left( \inferrule{ \inferrule*{ }{\seq{w:\mult{\rho_i}}{w}{\rho_i}} \sep
      \inferrule*{
        \seq{\dem {\Phi^i} ^i_{\lam z p}; z}{\N_i }{p}{\rho_i}}{
        \seq{ \Gam^i_{\lam z p}; z:\N_i }{p}{\mult{\rho_i}}}
      }{\inferrule*{\seq{\Gam^i_{\lam z p}; z:\N_i}{w \es w p}{
  \rho_i}}{\seq{\Gam^i_{\lam z p} }{\lam z w \es w p }{ \N_i \ft \rho_i}}} \right)_{\iI}}
      {\seq{\Gam_{\lam z p}}{\lam z w \es w p  }{ \M}}}
      {\seq{\Delta + \Gam_{\lam z p}}{t {\dist x {\lam z w \es w p}}}{ \tau}} \]
      We have
      \begin{align*}
        \dermeasaux{\Phi_{u_1}} m
        &= \dermeasaux{\Phi} m + \sum_{\iI} \left(\dermeasaux{\Phi^i}{m + \lv x t + 1} + (0,0,1) + (1,m+\lv x t,0)\right)< \dermeasaux{\Phi_{u_0}} m
      \end{align*}
      since $(1,m+\lv x t,1) < (1,m+\lv x t+1,0)$.
    \item $u_0 = \ctxnc\ictx x \dist x {\lam z {\ctx\llc p}} 
      \rrule\absrr^y \ctx\llc{\ctxnc\ictx{\lam z p}} = u_1$,
      where $z \notin \fv \llc$.
      By \autoref{l:sr_permlr}, there is a derivation
      $\dem {\Phi_{u_0}'} {\Gamma'}{\ctx\llc{\ctxnc\ictx x \dist x {\lam
      z p}}}{\tau}$
      such that $\dermeasaux {\Phi_{u_0}'} m = \dermeasaux {\Phi_{u_0}} m$.
      Let $\Phi''_{u_0}$ be the following subderivation of $\Phi_{u_0}'$.
      \[ \Phi''_{u_0} =
      \inferrule*[right=(\cuttr)]{
        \dem {\Phi} {\Delta; x:\M}{\ctxnc\ictx x}{\tau}
        \\ \dem {\Phi_p} {\Gamma_p}{\lam z p}{\M}}{
        \seq{\Delta + \Gamma_p}{\ctxnc\ictx x \dist x {\lam z p}}{\tau}}
      \]
      Then, by \autoref{l:partial-substitution} we have
      $\dem {\Phi_{u_1'}} {\Delta + \Gamma_p}{\ctxnc\ictx{\lam z p}}{\sigma}$,
      where $\dermeasaux{\Phi_{u_1}} m
      =_{\autoref{l:partial-substitution}} \dermeasaux \Phi m + \dermeasaux{\Phi_p}{m+d} - (0,0,\ssz\M)
      \leq \dermeasaux{\Phi_{u_0}''} m$.
      Hence, $\dermeasaux{\Phi_{u_1}} m \leq \dermeasaux{\Phi_{u_0}} m$.
  \end{itemize}

  Now we prove  weighted subject reduction for the contextual rules
  $\skctxtop$ and $\skctxdeep$.
  If $t_0 = \lam y {\ctx\llc t}
  \Rew\redsubw \lam y {\ctx\llc {t'}} = t_1$
  comes from $t \rrule{}^y t'$ (resp. $t_0 = \lam y {\ctx\llc{u \dist x t}}
  \Rew\redsubw \lam y {\ctx\llc{u \dist x {t'}}} = t_1$ comes from $t \Rew\redsubw t'$), then by construction 
  there is a subderivation $\dem {\Phi_t} {\Gamma'}{t}{\tau}$.
  By the proof of weighted subject reduction on $\rrule{}^y$ (resp. by the \ih),
  there is a derivation  $\dem {\Phi_{t'}} {\Gamma'}{t'}{\tau}$
  such that $\dermeasaux{\Phi_{t}} m \geq \dermeasaux{\Phi_{t'}} m$.
  We build $\Phi_{t_1}$ by replacing the derivation $\Phi_t$ by  $\Phi_{t'}$,
  we thus get $\Phi_{t_0} \geq \Phi_{t_1}$. 
\end{proof}


